A System Level Analysis for Integrated Sensing and Communication

In this work, we provide a system level analysis of integrated sensing and communication (ISAC) systems, where a setup with a mono-static dual-functional radar communication base station is assumed. We derive the ISAC signal-to-noise ratio (SNR) equation that relates communication and radar SNR for different distances. We also derive the ISAC range equation, which can be used for sensing-assisted beamforming applications. Specifically, we show that increasing the frequency and bandwidth is more favorable to the radar application in terms of relative SNR and range while increasing the transmit power is more favorable to communications. Numerical examples reveal that if the range for communication and radar is desired to be in the same order, the ISAC system should operate in mmWave or sub-THz bands, whereas sub-6GHz allows scenarios where the communication range is of orders of magnitude higher than that of radar.

==> figs/data_config1.tex <==
81.5582278139513	60.5661291737303\\
75.5376279006717	48.5249293471711\\
72.0158027195581	41.4812789849439\\
69.5170279873921	36.4837295206119\\
67.5788277272309	32.6073290002896\\
65.9952028062784	29.4400791583846\\
64.6562670136662	26.7622075731601\\
63.4964280741124	24.4425296940526\\
62.4733776251648	22.3964287961574\\
61.5582278139513	20.5661291737303\\
60.7303741107868	18.9104217674013\\
59.9746028929988	17.3988793318254\\
59.2793607678146	16.0083950814569\\
58.6356671003865	14.7210077466008\\
58.0364026328377	13.5224788115031\\
57.4758281608328	12.4013298674934\\
56.9492493863858	11.3481723185994\\
56.4527777118852	10.3552289695981\\
55.9831557948947	9.41598513561719\\
55.5376279006717	8.5249293471711\\
55.1138419192729	7.67735738437358\\
54.7097741975072	6.8692219408421\\
54.3236710935995	6.09701573302663\\
53.9540029797192	5.35767950526611\\
53.5994276405106	4.64852882684884\\
53.2587608545349	3.96719525489763\\
52.9309525307716	3.31157860737086\\
52.6150671871069	2.67980792004158\\
52.3102678559722	2.0702092577721\\
52.0158027195581	1.48127898494385\\
51.7309939372659	0.911661420359442\\
51.4552282475532	0.36013004093411\\
51.1879490163936	-0.17442842138515\\
50.9286494731062	-0.693027507959856\\
50.6768669269458	-1.19659260028068\\
50.4321777986056	-1.68597085696114\\
50.1941933326114	-2.16193978894945\\
49.9625558816151	-2.62521469094206\\
49.7369356734213	-3.07645510732962\\
49.5170279873921	-3.51627047938815\\
49.3025506795566	-3.94522509505907\\
49.0932420059933	-4.36384244218567\\
48.8888587023596	-4.77260904945311\\
48.6891742842276	-5.17197788571715\\
48.4939775384444	-5.5623713772834\\
48.3030711803198	-5.94418409353261\\
48.116270655237	-6.31778514369835\\
47.9334030664396	-6.68352032129314\\
47.754306213381	-7.0417140274102\\
47.5788277272309	-7.3926709997104\\
47.4068242919926	-7.7366778701871\\
47.2381609412553	-8.07400457166162\\
47.0727104219355	-8.40490561030121\\
46.9103526174919	-8.72962121918839\\
46.7509740240664	-9.0483784060394\\
46.5944672738273	-9.36139190651767\\
46.4407307005015	-9.66886505316931\\
46.2896679426926	-9.97099056878714\\
46.1411875811084	-10.2679512919554\\
45.9952028062784	-10.5599208416154\\
45.851631113736	-10.8470642267003\\
45.7103940239862	-11.1295384061998\\
45.5714168248797	-11.4074928044129\\
45.4346283342736	-11.6810697856251\\
45.2999606810942	-11.9504050919839\\
45.1673491031139	-12.2156282479444\\
45.0367317599348	-12.4768629343027\\
44.9080495598266	-12.7342273345191\\
44.7812459992062	-12.9878344557599\\
44.6562670136662	-13.2377924268399\\
44.5330608395698	-13.4842047750327\\
44.4115778853259	-13.7271706835204\\
44.2917706115422	-13.9667852310879\\
44.1735934193318	-14.2031396155087\\
44.0570025461173	-14.4363213619377\\
43.9419559683355	-14.6664145175013\\
43.8284133105017	-14.8934998331689\\
43.7163357601417	-15.1176549338889\\
43.6056859881425	-15.3389544778873\\
43.4964280741124	-15.5574703059474\\
43.3885274363783	-15.7732715814156\\
43.281950766277	-15.9864249216183\\
43.1766659664298	-16.1969945213126\\
43.0726420927137	-16.4050422687449\\
42.9698492996655	-16.6106278548414\\
42.86825878908	-16.8138088760124\\
42.7678427615789	-17.0146409310144\\
42.6685743709479	-17.2131777122764\\
42.5704276810531	-17.4094710920662\\
42.4733776251648	-17.6035712038426\\
42.3773999675294	-17.7955265191134\\
42.2824712670402	-17.9853839200919\\
42.1885688428726	-18.1731887684271\\
42.0956707419573	-18.3589849702576\\
42.0037557081744	-18.5428150378236\\
41.9128031531599	-18.7247201478524\\
41.8227931286264	-18.9047401969194\\
41.7337063001014	-19.0829138539694\\
41.6455239220003	-19.2592786101716\\
41.5582278139513	-19.4338708262697\\
41.4718003382985	-19.6067257775754\\
41.386224378713	-19.7778776967464\\
41.3014833198479	-19.9473598144765\\
41.2175610279757	-20.1152043982209\\
41.1344418325525	-20.2814427890672\\
41.0521105086559	-20.4461054368605\\
40.9705522602471	-20.609221933678\\
40.8897527042123	-20.7708210457476\\
40.8096978551388	-20.9309307438946\\
40.7303741107868	-21.0895782325987\\
40.6517682382182	-21.2467899777359\\
40.5738673605477	-21.4025917330769\\
40.4966589442829	-21.5570085656064\\
40.4201307872219	-21.7100648797286\\
40.3442710068791	-21.8617844404141\\
40.2690680294129	-22.0121903953464\\
40.1945105790281	-22.1613052961161\\
40.1205876678288	-22.3091511185147\\
40.0472885861007	-22.4557492819709\\
39.9746028929988	-22.6011206681746\\
39.9025204076223	-22.7452856389277\\
39.8310312004563	-22.8882640532596\\
39.7601255851634	-23.0300752838456\\
39.6897941107066	-23.1707382327591\\
39.6200275537902	-23.3102713465919\\
39.5508169116001	-23.4486926309722\\
39.4821533948322	-23.5860196645079\\
39.4140284209939	-23.7222696121844\\
39.3464336079663	-23.8574592382396\\
39.2793607678146	-23.9916049185431\\
39.212801900836	-24.1247226525002\\
39.1467491898343	-24.2568280745036\\
39.0811949946096	-24.3879364649531\\
39.0161318466552	-24.518062760862\\
38.9515524440512	-24.6472215660699\\
38.887449646547	-24.7754271610783\\
38.8238164708232	-24.9026935125259\\
38.7606460859266	-25.0290342823191\\
38.6979318088694	-25.1544628364335\\
38.6356671003865	-25.2789922533992\\
38.5738455608437	-25.4026353324848\\
38.5124609262902	-25.5254046015919\\
38.4515070646501	-25.6473123248721\\
38.3909779720463	-25.7683705100796\\
38.3308677692518	-25.8885909156686\\
38.2711706982626	-26.0079850576471\\
38.2118811189878	-26.1265642161967\\
38.1529935060522	-26.2443394420679\\
38.0945024457058	-26.3613215627606\\
38.0364026328377	-26.4775211884969\\
37.9786888680879	-26.5929487179964\\
37.9213560550559	-26.7076143440606\\
37.8643991975993	-26.8215280589736\\
37.807813397222	-26.9346996597282\\
37.7515938505455	-27.0471387530813\\
37.6957358468621	-27.1588547604481\\
37.6402347657666	-27.269856922639\\
37.5850860748629	-27.3801543044466\\
37.5302853275423	-27.4897557990877\\
37.4758281608328	-27.5986701325066\\
37.4217102933143	-27.7069058675436\\
37.3679275230987	-27.8144714079749\\
37.3144757258722	-27.921375002428\\
37.2613508529974	-28.0276247481776\\
37.2085489296732	-28.1332285948259\\
37.1560660531502	-28.2381943478719\\
37.1038983909996	-28.342529672173\\
37.0520421794341	-28.4462420953042\\
37.0004937216778	-28.5493390108166\\
36.9492493863858	-28.6518276814006\\
36.8983056061082	-28.7537152419558\\
36.8476588758003	-28.8550087025716\\
36.7973057513754	-28.9557149514215\\
36.7472428482993	-29.0558407575736\\
36.6974668402254	-29.1553927737214\\
36.6479744576683	-29.2543775388356\\
36.5987624867152	-29.3528014807419\\
36.5498277677734	-29.4506709186254\\
36.5011671943534	-29.5479920654654\\
36.4527777118852	-29.6447710304019\\
36.4046563165676	-29.741013821037\\
36.3568000542498	-29.8367263456726\\
36.3092060193427	-29.9319144154868\\
36.2618713537606	-30.0265837466511\\
36.214793245891	-30.1207399623902\\
36.167968929593	-30.2143885949863\\
36.1213956832213	-30.3075350877296\\
36.0750708286777	-30.4001847968168\\
36.0289917304864	-30.4923429931994\\
35.9831557948947	-30.5840148643828\\
35.9375604689968	-30.6752055161788\\
35.8922032398803	-30.7659199744116\\
35.8470816337958	-30.8561631865806\\
35.8021932153468	-30.9459400234787\\
35.7575355867009	-31.0352552807704\\
35.7131063868218	-31.1241136805287\\
35.6689032907194	-31.2125198727334\\
35.6249240087207	-31.3004784367309\\
35.5811662857572	-31.3879938826579\\
35.5376279006717	-31.4750706528289\\
35.4943066655415	-31.5617131230892\\
35.4512004250188	-31.6479256041346\\
35.4083070556871	-31.7337123427982\\
35.3656244654333	-31.8190775233056\\
35.3231505928362	-31.9040252684998\\
35.2808834065682	-31.9885596410358\\
35.238820904813	-32.0726846445464\\
35.1969611146961	-32.1564042247801\\
35.1553020917302	-32.2397222707118\\
35.1138419192729	-32.3226426156264\\
35.0725787079975	-32.4051690381774\\
35.0315105953763	-32.4873052634197\\
34.9906357451766	-32.5690549638192\\
34.9499523469675	-32.6504217602373\\
34.9094586156392	-32.7314092228939\\
34.8691527909327	-32.8120208723069\\
34.8290331369807	-32.8922601802108\\
34.7890979418592	-32.9721305704538\\
34.7493455171489	-33.0516354198744\\
34.7097741975072	-33.1307780591579\\
34.6703823402491	-33.2095617736741\\
34.6311683249385	-33.2879898042952\\
34.5921305529881	-33.3660653481961\\
34.5532674472681	-33.4437915596362\\
34.5145774517241	-33.5211715507241\\
34.4760590310033	-33.5982083921657\\
34.4377106700889	-33.6749051139946\\
34.3995308739422	-33.7512647062878\\
34.3615181671535	-33.8272901198652\\
34.3236710935995	-33.9029842669734\\
34.2859882161084	-33.9783500219554\\
34.2484681161333	-34.0533902219056\\
34.2111093934309	-34.1281076673104\\
34.1739106657485	-34.2025051226754\\
34.1368705685166	-34.2765853171391\\
34.0999877545492	-34.3503509450739\\
34.0632608937492	-34.4238046666738\\
34.0266886728211	-34.4969491085301\\
33.9902697949886	-34.5697868641952\\
33.9540029797192	-34.6423204947339\\
33.9178869624539	-34.7145525292644\\
33.8819204943427	-34.7864854654869\\
33.8461023419851	-34.8581217702021\\
33.8104312871767	-34.9294638798188\\
33.7749061266607	-35.000514200851\\
33.7395256718837	-35.0712751104048\\
33.704288748758	-35.1417489566563\\
33.669194197427	-35.2119380593183\\
33.6342408720366	-35.2818447100991\\
33.5994276405106	-35.3514711731512\\
33.5647533843305	-35.4208196855112\\
33.5302169983204	-35.4898924575314\\
33.495817390435	-35.5586916733024\\
33.4615534815525	-35.6272194910672\\
33.4274242052722	-35.6954780436279\\
33.3934285077143	-35.7634694387436\\
33.3595653473254	-35.8311957595214\\
33.3258336946867	-35.8986590647989\\
33.2922325323263	-35.9658613895197\\
33.2587608545349	-36.0328047451024\\
33.2254176671857	-36.0994911198009\\
33.1922019875564	-36.1659224790595\\
33.1591128441562	-36.23210076586\\
33.1261492765547	-36.2980279010629\\
33.0933103352152	-36.363705783742\\
33.06059508133	-36.4291362915123\\
33.0280025866598	-36.4943212808527\\
32.9955319333755	-36.5592625874212\\
32.9631822139032	-36.623962026366\\
32.9309525307716	-36.6884213926291\\
32.8988419964632	-36.7526424612459\\
32.8668497332673	-36.8166269876376\\
32.8349748731362	-36.8803767078999\\
32.8032165575435	-36.9438933390852\\
32.7715739373461	-37.0071785794802\\
32.740046172647	-37.0702341088784\\
32.7086324326623	-37.1330615888476\\
32.6773318955898	-37.1956626629927\\
32.6461437484794	-37.2580389572136\\
32.6150671871069	-37.3201920799584\\
32.5841014158497	-37.3821236224728\\
32.5532456475641	-37.4438351590441\\
32.5224991034655	-37.5053282472413\\
32.4918610130106	-37.5666044281512\\
32.4613306137811	-37.6276652266101\\
32.4309071513704	-37.6885121514314\\
32.4005898792715	-37.7491466956293\\
32.3703780587667	-37.8095703366389\\
32.3402709588204	-37.8697845365316\\
32.3102678559722	-37.9297907422279\\
32.2803680342332	-37.9895903857059\\
32.2505707849829	-38.0491848842064\\
32.2208754068691	-38.108575640434\\
32.1912812057082	-38.1677640427559\\
32.1617874943881	-38.2267514653962\\
32.1323935927725	-38.2855392686272\\
32.1030988276071	-38.3441287989581\\
32.0739025324262	-38.4025213893199\\
32.0448040474627	-38.4607183592468\\
32.0158027195581	-38.5187210150561\\
31.9868979020744	-38.5765306500234\\
31.9580889548083	-38.6341485445557\\
31.9293752439052	-38.6915759663619\\
31.9007561417762	-38.7488141706198\\
31.8722310270156	-38.8058644001411\\
31.8437992843197	-38.8627278855328\\
31.8154603044076	-38.9194058453571\\
31.7872134839424	-38.9758994862874\\
31.7590582254546	-39.032210003263\\
31.7309939372659	-39.0883385796406\\
31.7030200334146	-39.1442863873432\\
31.6751359335825	-39.2000545870074\\
31.6473410630223	-39.2556443281276\\
31.619634852487	-39.3110567491983\\
31.5920167381593	-39.3662929778537\\
31.5644861615832	-39.4213541310058\\
31.5370425695963	-39.4762413149797\\
31.5096854142627	-39.530955625647\\
31.4824141528077	-39.5854981485569\\
31.4552282475532	-39.6398699590659\\
31.4281271658539	-39.6940721224645\\
31.4011103800347	-39.7481056941029\\
31.3741773673293	-39.8019717195138\\
31.3473276098191	-39.8556712345341\\
31.3205605943738	-39.9092052654246\\
31.2938758125925	-39.9625748289872\\
31.2672727607456	-40.0157809326811\\
31.2407509397177	-40.0688245747368\\
31.2143098549518	-40.1217067442686\\
31.1879490163936	-40.1744284213852\\
31.1616679384369	-40.2269905772984\\
31.1354661398706	-40.2793941744311\\
31.1093431438249	-40.3316401665224\\
31.08329847772	-40.3837294987322\\
31.0573316732144	-40.4356631077435\\
31.0314422661544	-40.4874419218634\\
31.0056297965245	-40.5390668611232\\
30.9798938083982	-40.5905388373758\\
30.9542338498897	-40.6418587543929\\
30.9286494731062	-40.6930275079599\\
30.9031402341014	-40.7440459859696\\
30.8777056928286	-40.7949150685151\\
30.8523454130959	-40.8456356279805\\
30.8270589625207	-40.8962085291309\\
30.8018459124858	-40.9466346292006\\
30.7767058380958	-40.9969147779807\\
30.7516383181338	-41.0470498179046\\
30.7266429350197	-41.0970405841329\\
30.7017192747677	-41.1468879046368\\
30.6768669269458	-41.1965926002807\\
30.6520854846348	-41.2461554849026\\
30.6273745443887	-41.2955773653949\\
30.6027337061949	-41.3448590417826\\
30.5781625734356	-41.3940013073012\\
30.5536607528494	-41.4430049484734\\
30.5292278544938	-41.4918707451847\\
30.5048634917074	-41.5405994707574\\
30.4805672810738	-41.5891918920246\\
30.4563388423849	-41.6376487694024\\
30.4321777986056	-41.6859708569611\\
30.4080837758382	-41.734158902496\\
30.384056403288	-41.7822136475963\\
30.3600953132291	-41.8301358277142\\
30.3362001409702	-41.8779261722319\\
30.3123705248218	-41.9255854045286\\
30.2886061060631	-41.9731142420461\\
30.2649065289095	-42.0205133963532\\
30.241271440481	-42.0677835732104\\
30.2177004907701	-42.1149254726321\\
30.1941933326114	-42.1619397889495\\
30.1707496216504	-42.2088272108715\\
30.1473690163134	-42.2555884215456\\
30.1240511777776	-42.3022240986172\\
30.1007957699417	-42.3487349142889\\
30.0776024593969	-42.3951215353784\\
30.0544709153981	-42.4413846233761\\
30.0314008098355	-42.4875248345014\\
30.0083918172068	-42.5335428197587\\
29.9854436145899	-42.5794392249925\\
29.9625558816151	-42.6252146909421\\
29.9397283004389	-42.6708698532944\\
29.9169605557171	-42.716405342738\\
29.8942523345789	-42.7618217850146\\
29.8716033266007	-42.8071198009709\\
29.8490132237813	-42.8523000066097\\
29.8264817205162	-42.8973630131399\\
29.8040085135731	-42.9423094270261\\
29.7815933020672	-42.9871398500379\\
29.7592357874372	-43.031854879298\\
29.7369356734213	-43.0764551073296\\
29.714692666034	-43.1209411221043\\
29.6925064735422	-43.1653135070879\\
29.6703768064428	-43.2095728412867\\
29.6483033774398	-43.2537196992926\\
29.6262859014221	-43.2977546513281\\
29.6043240954411	-43.3416782632901\\
29.582417678689	-43.3854910967943\\
29.5605663724776	-43.4291937092172\\
29.5387699002163	-43.4727866537396\\
29.5170279873921	-43.5162704793881\\
29.4953403615477	-43.5596457310769\\
29.4737067522619	-43.6029129496485\\
29.4521268911291	-43.646072671914\\
29.4306005117392	-43.6891254306938\\
29.4091273496579	-43.7320717548564\\
29.3877071424074	-43.7749121693574\\
29.3663396294469	-43.8176471952784\\
29.3450245521537	-43.8602773498649\\
29.3237616538045	-43.9028031465633\\
29.3025506795566	-43.9452250950591\\
29.2813913764299	-43.9875437013124\\
29.2602834932886	-44.029759467595\\
29.2392267808233	-44.0718728925257\\
29.2182209915333	-44.1138844711056\\
29.1972658797095	-44.1557946947534\\
29.1763612014165	-44.1976040513394\\
29.1555067144762	-44.23931302522\\
29.1347021784506	-44.2809220972711\\
29.1139473546254	-44.3224317449215\\
29.0932420059933	-44.3638424421857\\
29.0725858972379	-44.4051546596964\\
29.0519787947178	-44.4463688647366\\
29.0314204664505	-44.4874855212713\\
29.0109106820967	-44.528505089979\\
28.9904492129451	-44.5694280282821\\
28.9700358318969	-44.6102547903784\\
28.9496703134508	-44.6509858272706\\
28.9293524336879	-44.6916215867965\\
28.9090819702568	-44.7321625136586\\
28.8888587023596	-44.7726090494531\\
28.8686824107367	-44.8129616326989\\
28.8485528776531	-44.8532206988661\\
28.828469886884	-44.8933866804043\\
28.8084332237011	-44.9334600067701\\
28.7884426748586	-44.9734411044551\\
28.7684980285796	-45.0133303970131\\
28.7485990745429	-45.0531283050865\\
28.7287456038693	-45.0928352464336\\
28.7089374091089	-45.1324516359545\\
28.6891742842276	-45.1719778857171\\
28.6694560245945	-45.2114144049832\\
28.6497824269695	-45.2507616002333\\
28.6301532894899	-45.2900198751924\\
28.6105684116589	-45.3291896308544\\
28.5910275943327	-45.3682712655069\\
28.5715306397085	-45.4072651747553\\
28.5520773513126	-45.4461717515471\\
28.5326675339884	-45.4849913861954\\
28.5133009938848	-45.5237244664026\\
28.4939775384444	-45.5623713772834\\
28.4746969763921	-45.6009325013881\\
28.4554591177237	-45.6394082187249\\
28.4362637736947	-45.6777989067829\\
28.4171107568092	-45.7161049405538\\
28.3979998808091	-45.7543266925541\\
28.3789309606626	-45.792464532847\\
28.3599038125543	-45.8305188290637\\
28.3409182538739	-45.8684899464244\\
28.3219741032061	-45.9063782477601\\
28.3030711803198	-45.9441840935326\\
28.2842093061583	-45.9819078418556\\
28.2653883028288	-46.0195498485147\\
28.2466079935922	-46.0571104669878\\
28.2278682028537	-46.0945900484649\\
28.2091687561522	-46.1319889418678\\
28.1905094801513	-46.1693074938697\\
28.1718902026291	-46.2065460489141\\
28.1533107524688	-46.2437049492346\\
28.1347709596496	-46.280784534873\\
28.116270655237	-46.3177851436984\\
28.0978096713734	-46.3547071114255\\
28.0793878412696	-46.3915507716332\\
28.0610049991951	-46.4283164557821\\
28.0426609804696	-46.4650044932331\\
28.024355621454	-46.5016152112643\\
28.0060887595414	-46.5381489350894\\
27.987860233149	-46.5746059878742\\
27.9696698817089	-46.6109866907544\\
27.95151754566	-46.6472913628522\\
27.9334030664396	-46.6835203212931\\
27.9153262864747	-46.7196738812229\\
27.8972870491743	-46.7557523558236\\
27.8792851989211	-46.7917560563301\\
27.8613205810631	-46.8276852920461\\
27.843393041906	-46.8635403703602\\
27.8255024287054	-46.8993215967614\\
27.8076485896586	-46.935029274855\\
27.7898313738971	-46.9706637063781\\
27.7720506314789	-47.0062251912145\\
27.754306213381	-47.0417140274102\\
27.7365979714919	-47.0771305111884\\
27.7189257586041	-47.1124749369641\\
27.7012894284067	-47.1477475973589\\
27.6836888354784	-47.1829487832155\\
27.6661238352799	-47.2180787836124\\
27.6485942841474	-47.2531378858775\\
27.6311000392847	-47.2881263756029\\
27.613640958757	-47.3230445366583\\
27.5962169014835	-47.3578926512052\\
27.5788277272309	-47.3926709997104\\
27.5614732966064	-47.4273798609595\\
27.5441534710509	-47.4620195120704\\
27.5268681128328	-47.4965902285067\\
27.5096170850408	-47.5310922840907\\
27.4924002515781	-47.5655259510161\\
27.4752174771553	-47.5998914998616\\
27.4580686272846	-47.6341891996031\\
27.4409535682729	-47.6684193176264\\
27.4238721672161	-47.70258211974\\
27.4068242919926	-47.7366778701871\\
27.3898098112571	-47.7707068316582\\
27.3728285944347	-47.8046692653029\\
27.355880511715	-47.8385654307423\\
27.3389654340458	-47.8723955860807\\
27.3220832331275	-47.9061599879173\\
27.3052337814071	-47.9398588913581\\
27.2884169520725	-47.9734925500274\\
27.2716326190466	-48.007061216079\\
27.2548806569822	-48.040565140208\\
27.2381609412553	-48.0740045716616\\
27.2214733479608	-48.1073797582506\\
27.2048177539061	-48.1406909463601\\
27.1881940366058	-48.1739383809606\\
27.1716020742768	-48.2071223056187\\
27.1550417458322	-48.2402429625079\\
27.1385129308765	-48.2733005924192\\
27.1220155097004	-48.3062954347715\\
27.1055493632751	-48.3392277276221\\
27.0891143732476	-48.3720977076771\\
27.0727104219355	-48.4049056103012\\
27.0563373923219	-48.4376516695284\\
27.0399951680503	-48.4703361180716\\
27.0236836334199	-48.5029591873325\\
27.0074026733802	-48.5355211074119\\
26.9911521735267	-48.5680221071188\\
26.9749320200959	-48.6004624139805\\
26.9587420999602	-48.6328422542519\\
26.9425823006235	-48.6651618529252\\
26.9264525102165	-48.6974214337392\\
26.9103526174919	-48.7296212191884\\
26.8942825118199	-48.7617614305324\\
26.8782420831836	-48.7938422878051\\
26.8622312221744	-48.8258640098235\\
26.8462498199877	-48.8578268141968\\
26.8302977684185	-48.8897309173353\\
26.8143749598566	-48.9215765344591\\
26.7984812872827	-48.9533638796069\\
26.7826166442639	-48.9850931656444\\
26.7667809249495	-49.0167646042733\\
26.7509740240664	-49.0483784060394\\
26.7351958369156	-49.079934780341\\
26.7194462593673	-49.1114339354376\\
26.7037251878573	-49.1428760784576\\
26.6880325193827	-49.1742614154068\\
26.6723681514978	-49.2055901511767\\
26.6567319823102	-49.236862489552\\
26.6411239104767	-49.2680786332188\\
26.6255438351997	-49.2992387837728\\
26.6099916562228	-49.3303431417266\\
26.5944672738273	-49.3613919065177\\
26.5789705888281	-49.3923852765161\\
26.5635015025701	-49.4233234490321\\
26.5480599169244	-49.4542066203235\\
26.5326457342845	-49.4850349856033\\
26.5172588575625	-49.5158087390472\\
26.5018991901859	-49.5465280738005\\
26.4865666360932	-49.5771931819859\\
26.4712610997309	-49.6078042547104\\
26.4559824860499	-49.6383614820725\\
26.4407307005015	-49.6688650531693\\
26.4255056490343	-49.6993151561036\\
26.4103072380908	-49.7297119779906\\
26.3951353746035	-49.7600557049653\\
26.3799899659918	-49.7903465221886\\
26.3648709201587	-49.8205846138549\\
26.3497781454871	-49.8507701631981\\
26.3347115508367	-49.8809033524989\\
26.3196710455407	-49.9109843630908\\
26.3046565394026	-49.9410133753671\\
26.2896679426926	-49.9709905687871\\
26.2747051661447	-50.0009161218829\\
26.2597681209535	-50.0307902122652\\
26.244856718771	-50.0606130166302\\
26.2299708717033	-50.0903847107656\\
26.2151104923077	-50.1201054695569\\
26.2002754935895	-50.1497754669933\\
26.185465788999	-50.1793948761742\\
26.1706812924285	-50.2089638693152\\
26.1559219182093	-50.2384826177537\\
26.1411875811084	-50.2679512919554\\
26.1264781963262	-50.2973700615199\\
26.1117936794929	-50.3267390951864\\
26.0971339466661	-50.3560585608402\\
26.0824989143274	-50.3853286255174\\
26.0678884993803	-50.4145494554116\\
26.0533026191466	-50.4437212158791\\
26.0387411913639	-50.4728440714444\\
26.0242041341831	-50.5019181858061\\
26.0096913661651	-50.5309437218421\\
25.9952028062784	-50.5599208416154\\
25.9807383738965	-50.5888497063792\\
25.9662979887948	-50.6177304765826\\
25.9518815711483	-50.6465633118757\\
25.9374890415287	-50.6753483711149\\
25.9231203209019	-50.7040858123684\\
25.9087753306256	-50.7327757929211\\
25.8944539924462	-50.76141846928\\
25.8801562284966	-50.790013997179\\
25.8658819612938	-50.8185625315847\\
25.851631113736	-50.8470642267003\\
25.8374036091002	-50.8755192359718\\
25.8231993710401	-50.9039277120921\\
25.809018323583	-50.9322898070063\\
25.794860391128	-50.9606056719164\\
25.780725498443	-50.9888754572863\\
25.7666135706628	-51.0170993128467\\
25.7525245332865	-51.0452773875993\\
25.738458312175	-51.0734098298223\\
25.724414833549	-51.1014967870744\\
25.7103940239862	-51.1295384061998\\
25.6963958104197	-51.1575348333329\\
25.6824201201349	-51.1854862139024\\
25.6684668807679	-51.2133926926364\\
25.6545360203028	-51.2412544135666\\
25.6406274670698	-51.2690715200327\\
25.6267411497427	-51.2968441546868\\
25.612876997337	-51.3245724594983\\
25.5990349392074	-51.3522565757575\\
25.5852149050459	-51.3798966440804\\
25.5714168248797	-51.4074928044129\\
25.5576406290686	-51.435045196035\\
25.5438862483036	-51.462553957565\\
25.5301536136042	-51.4900192269639\\
25.5164426563167	-51.517441141539\\
25.5027533081118	-51.5448198379487\\
25.489085500983	-51.5721554522062\\
25.4754391672443	-51.5994481196837\\
25.4618142395281	-51.6266979751161\\
25.4482106507833	-51.6539051526057\\
25.4346283342736	-51.6810697856251\\
25.421067223575	-51.7081920070223\\
25.4075272525742	-51.7352719490238\\
25.3940083554669	-51.7623097432385\\
25.3805104667551	-51.7893055206621\\
25.367033521246	-51.8162594116804\\
25.3535774540496	-51.843171546073\\
25.3401422005773	-51.8700420530177\\
25.3267276965394	-51.8968710610934\\
25.3133338779439	-51.9236586982844\\
25.2999606810942	-51.9504050919839\\
25.2866080425875	-51.9771103689973\\
25.2732758993129	-52.0037746555465\\
25.2599641884498	-52.0303980772726\\
25.246672847466	-52.0569807592403\\
25.2334018141157	-52.083522825941\\
25.2201510264381	-52.1100244012961\\
25.2069204227557	-52.1364856086609\\
25.1937099416722	-52.1629065708279\\
25.1805195220711	-52.18928741003\\
25.1673491031139	-52.2156282479444\\
25.1541986242385	-52.2419292056953\\
25.1410680251573	-52.2681904038576\\
25.1279572458558	-52.2944119624606\\
25.114866226591	-52.3205940009904\\
25.1017949078892	-52.3467366383938\\
25.0887432305453	-52.3728399930817\\
25.0757111356203	-52.3989041829316\\
25.0626985644404	-52.4249293252915\\
25.0497054585949	-52.4509155369826\\
25.0367317599348	-52.4768629343027\\
25.0237774105715	-52.5027716330293\\
25.0108423528748	-52.5286417484227\\
24.9979265294718	-52.5544733952287\\
24.9850298832449	-52.5802666876824\\
24.9721523573308	-52.6060217395106\\
24.9592938951186	-52.6317386639351\\
24.9464544402484	-52.6574175736754\\
24.93363393661	-52.6830585809522\\
24.9208323283413	-52.7086617974897\\
24.9080495598266	-52.7342273345191\\
24.8952855756956	-52.7597553027811\\
24.8825403208217	-52.7852458125288\\
24.8698137403207	-52.810698973531\\
24.857105779549	-52.8361148950743\\
24.8444163841028	-52.8614936859667\\
24.8317454998163	-52.8868354545397\\
24.8190930727603	-52.9121403086517\\
24.8064590492411	-52.9374083556901\\
24.7938433757988	-52.9626397025747\\
24.7812459992062	-52.9878344557599\\
24.7686668664673	-53.0129927212376\\
24.7561059248162	-53.03811460454\\
24.7435631217152	-53.0632002107419\\
24.7310384048542	-53.0882496444638\\
24.718531722149	-53.1132630098742\\
24.7060430217401	-53.1382404106921\\
24.6935722519911	-53.16318195019\\
24.6811193614881	-53.1880877311961\\
24.6686842990377	-53.2129578560969\\
24.6562670136662	-53.2377924268399\\
24.6438674546181	-53.262591544936\\
24.6314855713552	-53.2873553114619\\
24.6191213135548	-53.3120838270626\\
24.6067746311091	-53.3367771919541\\
24.5944454741233	-53.3614355059256\\
24.5821337929152	-53.3860588683418\\
24.5698395380133	-53.4106473781456\\
24.5575626601559	-53.4352011338604\\
24.54530311029	-53.4597202335923\\
24.5330608395698	-53.4842047750327\\
24.520835799356	-53.5086548554603\\
24.5086279412142	-53.5330705717439\\
24.496437216914	-53.5574520203443\\
24.4842635784278	-53.5817992973166\\
24.4721069779297	-53.6061124983129\\
24.4599673677942	-53.6303917185839\\
24.4478447005953	-53.6546370529817\\
24.4357389291053	-53.6788485959617\\
24.4236500062937	-53.703026441585\\
24.4115778853259	-53.7271706835204\\
24.3995225195627	-53.7512814150468\\
24.3874838625585	-53.7753587290552\\
24.3754618680607	-53.7994027180509\\
24.3634564900084	-53.8234134741555\\
24.3514676825314	-53.8473910891094\\
24.3394953999494	-53.8713356542734\\
24.3275395967706	-53.8952472606312\\
24.3156002276906	-53.9191259987911\\
24.3036772475918	-53.9429719589886\\
24.2917706115422	-53.9667852310879\\
24.2798802747941	-53.9905659045841\\
24.2680061927835	-54.0143140686053\\
24.2561483211287	-54.0380298119148\\
24.2443066156299	-54.0617132229125\\
24.2324810322674	-54.0853643896374\\
24.2206715272013	-54.1089833997696\\
24.2088780567703	-54.1325703406317\\
24.1971005774905	-54.1561252991913\\
24.1853390460548	-54.1796483620627\\
24.1735934193318	-54.2031396155087\\
24.1618636543647	-54.2265991454428\\
24.1501497083708	-54.2500270374307\\
24.1384515387398	-54.2734233766927\\
24.1267691030337	-54.2967882481048\\
24.1151023589855	-54.3201217362014\\
24.1034512644979	-54.3434239251764\\
24.0918157776433	-54.3666948988856\\
24.0801958566621	-54.3899347408481\\
24.068591459962	-54.4131435342483\\
24.0570025461173	-54.4363213619377\\
24.0454290738679	-54.4594683064364\\
24.0338710021185	-54.4825844499353\\
24.0223282899373	-54.5056698742977\\
24.0108008965558	-54.5287246610606\\
23.9992887813675	-54.5517488914372\\
23.9877919039272	-54.5747426463179\\
23.9763102239499	-54.5977060062726\\
23.9648437013102	-54.6206390515518\\
23.9533922960417	-54.6435418620889\\
23.9419559683355	-54.6664145175013\\
23.9305346785399	-54.6892570970926\\
23.9191283871593	-54.7120696798537\\
23.9077370548537	-54.7348523444649\\
23.8963606424375	-54.7576051692972\\
23.884999110879	-54.7803282324144\\
23.8736524212992	-54.8030216115738\\
23.8623205349717	-54.8256853842289\\
23.8510034133211	-54.8483196275301\\
23.8397010179227	-54.8709244183269\\
23.8284133105017	-54.8934998331689\\
23.8171402529322	-54.9160459483079\\
23.8058818072366	-54.9385628396991\\
23.7946379355848	-54.9610505830027\\
23.7834086002935	-54.9835092535854\\
23.7721937638251	-55.0059389265221\\
23.7609933887875	-55.0283396765972\\
23.749807437933	-55.0507115783062\\
23.7386358741575	-55.0730547058572\\
23.7274786605	-55.0953691331722\\
23.7163357601417	-55.1176549338889\\
23.7052071364053	-55.1399121813617\\
23.6940927527544	-55.1621409486636\\
23.6829925727924	-55.1843413085874\\
23.6719065602625	-55.2065133336472\\
23.6608346790463	-55.2286570960798\\
23.6497768931632	-55.250772667846\\
23.63873316677	-55.2728601206322\\
23.6277034641602	-55.2949195258519\\
23.6166877497629	-55.3169509546465\\
23.6056859881425	-55.3389544778873\\
23.5946981439978	-55.3609301661767\\
23.5837241821614	-55.3828780898494\\
23.5727640675992	-55.4047983189738\\
23.5618177654094	-55.4266909233535\\
23.5508852408219	-55.4485559725285\\
23.5399664591979	-55.4703935357764\\
23.5290613860291	-55.4922036821141\\
23.5181699869367	-55.5139864802988\\
23.5072922276715	-55.5357419988293\\
23.4964280741124	-55.5574703059474\\
23.4855774922666	-55.5791714696392\\
23.474740448268	-55.6008455576362\\
23.4639169083777	-55.6224926374169\\
23.4531068389823	-55.6441127762077\\
23.4423102065939	-55.6657060409844\\
23.4315269778495	-55.6872724984733\\
23.4207571195099	-55.7088122151525\\
23.4100005984596	-55.7303252572531\\
23.3992573817059	-55.7518116907605\\
23.3885274363783	-55.7732715814156\\
23.3778107297282	-55.7947049947159\\
23.3671072291278	-55.8161119959167\\
23.3564169020699	-55.8374926500324\\
23.3457397161673	-55.8588470218377\\
23.3350756391518	-55.8801751758687\\
23.3244246388741	-55.9014771764241\\
23.313786683303	-55.9227530875663\\
23.3031617405248	-55.9440029731226\\
23.2925497787429	-55.9652268966864\\
23.281950766277	-55.9864249216183\\
23.2713646715625	-56.0075971110473\\
23.2607914631503	-56.0287435278717\\
23.2502311097059	-56.0498642347604\\
23.239683580009	-56.0709592941543\\
23.2291488429528	-56.0920287682667\\
23.2186268675437	-56.1130727190849\\
23.2081176229004	-56.1340912083715\\
23.1976210782537	-56.1550842976649\\
23.1871372029458	-56.1760520482806\\
23.1766659664298	-56.1969945213126\\
23.1662073382691	-56.2179117776341\\
23.1557612881368	-56.2388038778986\\
23.1453277858156	-56.2596708825412\\
23.1349068011965	-56.2805128517792\\
23.1244983042793	-56.3013298456137\\
23.114102265171	-56.3221219238303\\
23.1037186540861	-56.3428891460001\\
23.0933474413458	-56.3636315714807\\
23.0829885973773	-56.3843492594177\\
23.0726420927137	-56.4050422687449\\
23.0623078979931	-56.4257106581861\\
23.0519859839583	-56.4463544862556\\
23.0416763214565	-56.4669738112593\\
23.0313788814382	-56.4875686912959\\
23.0210936349575	-56.5081391842573\\
23.0108205531708	-56.5286853478306\\
23.0005596073372	-56.5492072394979\\
22.990310768817	-56.5697049165382\\
22.9800740090723	-56.5901784360278\\
22.9698492996655	-56.6106278548414\\
22.9596366122596	-56.6310532296532\\
22.9494359186173	-56.6514546169377\\
22.9392471906008	-56.6718320729706\\
22.9290704001712	-56.6921856538299\\
22.9189055193879	-56.7125154153966\\
22.9087525204082	-56.7328214133558\\
22.8986113754873	-56.7531037031976\\
22.8884820569772	-56.7733623402179\\
22.8783645373265	-56.7935973795193\\
22.86825878908	-56.8138088760124\\
22.8581647848782	-56.8339968844158\\
22.8480824974571	-56.8541614592582\\
22.8380118996471	-56.874302654878\\
22.8279529643734	-56.8944205254254\\
22.817905664655	-56.9145151248622\\
22.8078699736044	-56.9345865069635\\
22.7978458644271	-56.9546347253181\\
22.7878333104215	-56.9746598333293\\
22.777832284978	-56.9946618842163\\
22.7678427615789	-57.0146409310144\\
22.757864713798	-57.0345970265762\\
22.7478981153	-57.0545302235723\\
22.7379429398399	-57.0744405744924\\
22.7279991612632	-57.0943281316458\\
22.718066753505	-57.1141929471622\\
22.7081456905897	-57.1340350729929\\
22.6982359466305	-57.1538545609113\\
22.6883374958293	-57.1736514625138\\
22.6784503124759	-57.1934258292205\\
22.6685743709479	-57.2131777122764\\
22.6587096457104	-57.2329071627516\\
22.6488561113149	-57.2526142315424\\
22.6390137423999	-57.2722989693724\\
22.6291825136898	-57.2919614267926\\
22.6193623999948	-57.3116016541827\\
22.6095533762103	-57.3312197017517\\
22.5997554173168	-57.3508156195387\\
22.5899684983793	-57.3703894574137\\
22.580192594547	-57.3899412650782\\
22.5704276810531	-57.4094710920662\\
22.5606737332138	-57.4289789877446\\
22.5509307264289	-57.4484650013146\\
22.5411986361804	-57.4679291818115\\
22.531477438033	-57.4873715781064\\
22.5217671076331	-57.5067922389061\\
22.5120676207088	-57.5261912127547\\
22.5023789530695	-57.5455685480333\\
22.4927010806052	-57.5649242929618\\
22.4830339792867	-57.5842584955988\\
22.4733776251648	-57.6035712038426\\
22.4637319943701	-57.6228624654322\\
22.4540970631125	-57.6421323279473\\
22.4444728076812	-57.6613808388099\\
22.434859204444	-57.6806080452842\\
22.4252562298472	-57.6998139944778\\
22.415663860415	-57.7189987333422\\
22.4060820727494	-57.7381623086735\\
22.3965108435296	-57.7573047671131\\
22.386950149512	-57.7764261551484\\
22.3773999675294	-57.7955265191134\\
22.3678602744913	-57.8146059051896\\
22.358331047383	-57.8336643594063\\
22.3488122632653	-57.8527019276416\\
22.3393038992747	-57.8717186556229\\
22.3298059326223	-57.8907145889276\\
22.3203183405943	-57.9096897729837\\
22.3108411005509	-57.9286442530705\\
22.3013741899265	-57.9475780743194\\
22.2919175862291	-57.9664912817141\\
22.2824712670402	-57.9853839200919\\
22.2730352100143	-58.0042560341436\\
22.2636093928787	-58.0231076684148\\
22.2541937934331	-58.0419388673061\\
22.2447883895492	-58.0607496750739\\
22.2353931591707	-58.079540135831\\
22.2260080803126	-58.098310293547\\
22.2166331310614	-58.1170601920495\\
22.2072682895741	-58.1357898750241\\
22.1979135340785	-58.1544993860153\\
22.1885688428726	-58.1731887684271\\
22.1792341943245	-58.1918580655233\\
22.1699095668717	-58.2105073204289\\
22.1605949390213	-58.2291365761296\\
22.1512902893494	-58.2477458754734\\
22.141995596501	-58.2663352611704\\
22.1327108391892	-58.2849047757939\\
22.1234359961957	-58.3034544617808\\
22.11417104637	-58.3219843614322\\
22.1049159686291	-58.3404945169141\\
22.0956707419573	-58.3589849702576\\
22.0864353454062	-58.3774557633599\\
22.0772097580938	-58.3959069379847\\
22.0679939592047	-58.4143385357628\\
22.0587879279899	-58.4327505981924\\
22.0495916437661	-58.4511431666402\\
22.0404050859155	-58.4695162823414\\
22.0312282338858	-58.4878699864006\\
22.02206106719	-58.5062043197923\\
22.0129035654055	-58.5245193233614\\
22.0037557081744	-58.5428150378236\\
21.994617475203	-58.5610915037662\\
21.9854888462618	-58.5793487616486\\
21.9763698011848	-58.5975868518027\\
21.9672603198694	-58.6158058144335\\
21.9581603822764	-58.6340056896195\\
21.9490699684293	-58.6521865173137\\
21.9399890584144	-58.6703483373434\\
21.9309176323804	-58.6884911894114\\
21.921855670538	-58.7066151130962\\
21.9128031531599	-58.7247201478524\\
21.9037600605804	-58.7428063330115\\
21.894726373195	-58.7608737077822\\
21.8857020714606	-58.778922311251\\
21.8766871358947	-58.7969521823829\\
21.8676815470755	-58.8149633600214\\
21.8586852856414	-58.8329558828894\\
21.8496983322913	-58.8509297895897\\
21.8407206677834	-58.8688851186054\\
21.831752272936	-58.8868219083003\\
21.8227931286264	-58.9047401969194\\
21.8138432157912	-58.9226400225898\\
21.8049025154258	-58.9405214233206\\
21.7959710085843	-58.9583844370037\\
21.787048676379	-58.9762291014143\\
21.7781354999806	-58.9940554542111\\
21.7692314606175	-59.0118635329373\\
21.7603365395758	-59.0296533750206\\
21.7514507181993	-59.0474250177737\\
21.7425739778886	-59.0651784983952\\
21.7337063001014	-59.0829138539694\\
21.7248476663523	-59.1006311214676\\
21.7159980582123	-59.1183303377476\\
21.7071574573086	-59.1360115395551\\
21.6983258453245	-59.1536747635233\\
21.6895032039991	-59.1713200461741\\
21.6806895151271	-59.1889474239181\\
21.6718847605586	-59.2065569330551\\
21.6630889221987	-59.2241486097748\\
21.6543019820077	-59.2417224901568\\
21.6455239220003	-59.2592786101716\\
21.6367547242458	-59.2768170056807\\
21.6279943708677	-59.2943377124368\\
21.6192428440437	-59.3118407660849\\
21.610500126005	-59.3293262021622\\
21.6017661990368	-59.3467940560987\\
21.5930410454773	-59.3642443632176\\
21.5843246477182	-59.3816771587359\\
21.5756169882039	-59.3990924777645\\
21.5669180494317	-59.4164903553089\\
21.5582278139513	-59.4338708262697\\

==> power_different_coupling_levels.tex <==


\tikzstyle{block} = [draw, fill=white, rectangle, 
minimum height=3em, minimum width=3em]
\tikzstyle{block2} = [draw, fill=white, rectangle, 
minimum height=1em, minimum width=2.4em]

%\tikzstyle{sum} = [draw, fill=blue!20, circle, node distance=1cm]
\tikzstyle{multiplier} = [draw,circle,fill=blue!20,add={}{}{}{}] {} 
\tikzstyle{sum} = [draw,circle,scale=0.7,add2={}{}{}{}] {} 
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\newcommand\z{4.5}


\def\windup{
	\tikz[remember picture,overlay]{
		%		\draw (-1,0) -- (1,0)  (0,-0.6)--(0,0.6);
		\draw (-0.8,0) -- (0.8,0);
		\draw (-0.8,-0.4)--(-0.4,-0.4) -- (0.4,0.4) --(0.8,0.4);
}}

% The block diagram code is probably more verbose than necessary
\centering
\begin{tikzpicture}[auto, node distance=0cm,>=latex']
	%\begin{tikzpicture}[auto]
	
	
	\draw[->] (-0.2, 0) -- (5, 0) node[below] {$P_{\rm C}$};
	\draw[->] (0, -0.2) -- (0, 4.5) node[left] {$P_{\rm R}$};	
	
	\draw[scale=4, domain=0:1, smooth, variable=\x, black] plot ({\x}, {1-\x}) node[right,xshift = -0cm,yshift = 0.1cm] {\footnotesize $\beta = 0$}; % beta = 0
	\draw[scale=4, domain=0.25:1, smooth, variable=\x, black] plot ({\x}, {1+0.25-\x}) node[right,xshift = -0cm,yshift = 0cm] {\footnotesize $\beta = 0.25$}; % beta = 0.25
	\draw[scale=4, domain=0.5:1, smooth, variable=\x, black] plot ({\x}, {1+0.5-\x}) node[right,xshift = -0cm,yshift = 0cm] {\footnotesize $\beta = 0.5$}; % beta = 0.5
	\draw[scale=4, domain=0.75:1, smooth, variable=\x,black] plot ({\x}, {1+0.75-\x}) node[right,xshift = -0cm,yshift = 0cm] {\footnotesize $\beta = 0.75$}; % beta = 0.75
	\draw plot[only marks,mark size = 2,mark={o}] coordinates{(4,4)} node[right,xshift = -0cm,yshift = 0cm] {\footnotesize $\beta = 1$};	
	
	\draw plot[only marks,mark size = 1.5,mark={square*}] coordinates{(0,2*2)} node[right,xshift = -0cm,yshift = 0cm] {};	
	\draw plot[only marks,mark size = 1.5,mark={square*}] coordinates{(0.5*2,2*2)} node[right,xshift = -0cm,yshift = 0cm] {};	
	\draw plot[only marks,mark size = 1.5,mark={square*}] coordinates{(1*2,2*2)} node[right,xshift = -0cm,yshift = 0cm] {};	
	\draw plot[only marks,mark size = 1.5,mark={square*}] coordinates{(1.5*2,2*2)} node[right,xshift = -0cm,yshift = 0cm] {};			
	
	\draw plot[only marks,mark size = 2,mark={*}] coordinates{(1*2,1*2)} node[right,xshift = -0cm,yshift = 0cm] {};	
	\draw plot[only marks,mark size = 2,mark={*}] coordinates{(1.25*2,1.25*2)} node[right,xshift = -0cm,yshift = 0cm] {};	
	\draw plot[only marks,mark size = 2,mark={*}] coordinates{(1.5*2,1.5*2)} node[right,xshift = -0cm,yshift = 0cm] {};	
	\draw plot[only marks,mark size = 2,mark={*}] coordinates{(1.75*2,1.75*2)} node[right,xshift = -0cm,yshift = 0cm] {};	
	
	\draw plot[only marks,mark size = 2,mark={diamond*}] coordinates{(2*2,0)} node[right,xshift = -0cm,yshift = 0cm] {};	
	\draw plot[only marks,mark size = 2,mark={diamond*}] coordinates{(2*2,0.5*2)} node[right,xshift = -0cm,yshift = 0cm] {};	
	\draw plot[only marks,mark size = 2,mark={diamond*}] coordinates{(2*2,1*2)} node[right,xshift = -0cm,yshift = 0cm] {};	
	\draw plot[only marks,mark size = 2,mark={diamond*}] coordinates{(2*2,1.5*2)} node[right,xshift = -0cm,yshift = 0cm] {};	
	
	\draw plot[only marks,mark size = 1.5,mark={square*}] coordinates{(-0.2+0.5,4.7)} node[right,xshift = -0cm,yshift = 0cm] {\footnotesize $\alpha = 0$};	
	\draw plot[only marks,mark size = 2,mark={*}] coordinates{(-0.2+1.2+0.5,4.7)} node[right,xshift = -0cm,yshift = 0cm] {\footnotesize $\alpha = 0.5$};	
	\draw plot[only marks,mark size = 2,mark={diamond*}] coordinates{(-0.2+2.6+0.5,4.7)} node[right,xshift = -0cm,yshift = 0cm] {\footnotesize $\alpha = 1$};	
	
	\draw node[xshift=0cm,yshift=-0.35cm] {\small $0$} node[xshift=-0.3cm,yshift=-0cm] {\small $0$};
	\draw node[xshift=4cm,yshift=-0.3cm] {\small $P$} node[xshift=-0.3cm,yshift=4cm] {\small $P$};
	
	\draw[scale=4, domain=1:0, smooth, variable=\x, black,dashed] plot ({\x},0.75) node[xshift=-0.4cm] {\footnotesize $0.75P$};
	\draw[scale=4, domain=1:0, smooth, variable=\x, black,dashed] plot ({\x},0.5) node[xshift=-0.4cm] {\footnotesize $0.5P$};
	\draw[scale=4, domain=1:0, smooth, variable=\x, black,dashed] plot ({\x},0.25) node[xshift=-0.4cm] {\footnotesize $0.25P$};
	
\end{tikzpicture}



==> snr_matching_generalized_log.tex <==


\tikzstyle{block} = [draw, fill=white, rectangle, 
minimum height=3em, minimum width=3em]
\tikzstyle{block2} = [draw, fill=white, rectangle, 
minimum height=1em, minimum width=2.4em]

%\tikzstyle{sum} = [draw, fill=blue!20, circle, node distance=1cm]
\tikzstyle{multiplier} = [draw,circle,fill=blue!20,add={}{}{}{}] {} 
\tikzstyle{sum} = [draw,circle,scale=0.7,add2={}{}{}{}] {} 
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\newcommand\z{0}


\def\windup{
	\tikz[remember picture,overlay]{
		%		\draw (-1,0) -- (1,0)  (0,-0.6)--(0,0.6);
		\draw (-0.8,0) -- (0.8,0);
		\draw (-0.8,-0.4)--(-0.4,-0.4) -- (0.4,0.4) --(0.8,0.4);
}}

% The block diagram code is probably more verbose than necessary
\centering
\begin{tikzpicture}[auto, node distance=0cm,>=latex']
	%\begin{tikzpicture}[auto]
	
	
	
	\draw[->] (\z-0.2, 0) -- (5+\z, 0) node[below] {$\tilde{\rho}_{\rm C}$};
	\draw[->] (0+\z, -0.2) -- (0+\z, 4.3) node[left] {$\tilde{\rho}_{\rm R}$};	
	\draw[shift = {(\z+4,4)},scale=4, domain=0.1:0.9, variable=\x, black,samples=25] plot ({log10{\x}}, {log10{(1-\x)}}) node[right,xshift = -0cm,yshift = 0.1cm] {\footnotesize $\beta = 0$}; % beta = 0
	\draw[shift = {(\z+4,4)},scale=4, domain=0.25:0.999, variable=\x, black,samples=25] plot ({log10{\x}}, {log10{(1.25-\x)}}) node[right,xshift = -0cm,yshift = 0.1cm] {\footnotesize $\beta = 0.25$}; % beta = 0
	\draw[shift = {(\z+4,4)},scale=4, domain=0.5:0.999, variable=\x, black,samples=25] plot ({log10{\x}}, {log10{(1.5-\x)}}) node[right,xshift = -0cm,yshift = 0.1cm] {\footnotesize $\beta = 0.5$}; % beta = 0
	%	\draw[shift = {(\z+2,2)},scale=4, domain=0.75:0.99, variable=\x, black,samples=25] plot ({log10{\x}}, {log10{(1.75-\x)}}) node[right,xshift = -0cm,yshift = 0.1cm] {\footnotesize $\beta = 0$}; % beta = 0
	\draw [shift = {(\z+4,4)}] plot[only marks,mark size = 2,mark={o}] coordinates{(0,0)} node[right,xshift = -0cm,yshift = 0cm] {\footnotesize $\beta = 1$};	
	%	\draw plot[only marks,mark size = 2,mark={o}] coordinates{(2,2)} node[right,xshift = -0cm,yshift = 0cm] {\footnotesize $\beta = 1$};	
	
	\draw [shift = {(\z,0)}] node[xshift=-0.1cm,yshift=-0.35cm] {\small $-10$} node[xshift=-0.55cm,yshift=-0cm] {\small $-10$};
	\draw [shift = {(\z,0)}] node[xshift=4cm,yshift=-0.2cm] {\small $0$} node[xshift=-0.2cm,yshift=4cm] {\small $0$};
	\draw[shift = {(\z,0)},scale=4, domain=1:0, smooth, variable=\x, black,dashed] plot ({\x},1-0.301) node[xshift=-0.4cm] {\footnotesize -3.01};
	\draw[shift = {(\z,0)},scale=4, domain=1:0, smooth, variable=\x, black,dashed] plot ({\x},1-0.602) node[xshift=-0.4cm] {\footnotesize -6.02};
	
	\draw[shift = {(\z+2,0)},scale=1, domain=-0.25:2.3, variable=\x, black,samples=25,dash dot] plot (\x, 2*\x) node[above,xshift = -0.0cm,yshift = -0.0cm] {\footnotesize equation \eqref{eq:snr_RC}}; % beta = 0	
\end{tikzpicture}


